Gamma-ray burst taxonomy: looking for the third class on the spectral peak energy-duration plane in the rest frame

Two classes of Gamma-ray bursts (GRBs), corresponding to the short/hard and the long/soft events, with a putative intermediate class, are typically considered in the observer frame. However, when considering GRB characteristics in the cosmological rest frame, the boundary between the classes becomes blurred. The goal of this research is to check for the evidences of a third "intermediate" class of GRBs and investigate how the transformation from the observer to the rest frame affects the hardness-duration-based classification. We applied fits with skewed and non-skewed (symmetric) Gaussian and Student distributions to the sample of 409 GRBs with reliably measured redshifts to cluster the bursts on the hardness (Ep) - duration (T90) plane. We found that, based on AIC/BIC criteria, the statistically preferred number of clusters on the GRB rest-frame hardnesses-duration plane does not exceed two. We also assess the robustness of the clustering technique. We did not find any solid evidence of an intermediate GRB class on the rest-frame hardness-duration plane.

==> tables/table_T50_bat.tex <==
\begin{table}
\caption[]{Information criteria for the rest-frame hardness-$T_{50}$ duration distributions of the ``KW  \& BAT'' sample. 
The acceptable models are shown in red ($\Delta \textrm{IC}< 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:T50bat}

$$ 
\begin{tabular}{llrrrrr}
\hline
\noalign{\smallskip}
Statistics & Cl. & Sample & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & $w_i$ (BIC) \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

$\mathcal{N}$ & 1 & KW \& BAT & \textcolor{red}{0.2} & 0.272 & \textcolor{red}{0.0} & 0.947 \\
$\mathcal{N}$ & 2 & KW \& BAT & \textcolor{red}{1.4} & 0.149 & 19.9 & $<0.001$ \\
$\mathcal{N}$ & 3 & KW \& BAT & \textcolor{red}{0.0} & 0.301 & 37.2 & $<0.001$ \\
\hline
$\mathcal{SN}$ & 1 & KW \& BAT & 4.2 & 0.037 & 10.3 & 0.005 \\
$\mathcal{SN}$ & 2 & KW \& BAT & 5.1 & 0.023 & 36.0 & $<0.001$ \\
$\mathcal{SN}$ & 3 & KW \& BAT & 6.1 & 0.014 & 62.0 & $<0.001$ \\
\hline
$\mathcal{T}$ & 1 & KW \& BAT & \textcolor{blue}{3.1} & 0.064 & 6.0 & 0.047 \\
$\mathcal{T}$ & 2 & KW \& BAT & \textcolor{red}{1.8} & 0.122 & 23.4 & $<0.001$ \\
$\mathcal{T}$ & 3 & KW \& BAT & 13.0 & $<0.001$ & 53.3 & $<0.001$ \\
\hline
$\mathcal{ST}$ & 1 & KW \& BAT & 7.6 & 0.007 & 16.7 & $<0.001$ \\
$\mathcal{ST}$ & 2 & KW \& BAT & 8.0 & 0.006 & 42.1 & $<0.001$ \\
$\mathcal{ST}$ & 3 & KW \& BAT & 8.4 & 0.005 & 67.4 & $<0.001$ \\

\hline

\noalign{\smallskip}
\end{tabular}
$$ 
\end{table}

==> tables/table_T50_kw.tex <==
\begin{table}
\caption[]{Information criteria for the rest-frame hardness-$T_{50}$ duration distributions of the ``KW  trig'' sample. 
The acceptable models are shown in red ($\Delta \textrm{IC}< 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:T50kw}

$$ 
\begin{tabular}{llrrrrr}
\hline
\noalign{\smallskip}
Statistics & Cl. & Sample & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & $w_i$ (BIC) \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

$\mathcal{N}$ & 1 & KW trig & 13.4 & $<0.001$ & 6.9 & 0.029 \\
$\mathcal{N}$ & 2 & KW trig & \textcolor{blue}{3.7} & 0.056 & 16.8 & $<0.001$ \\
$\mathcal{N}$ & 3 & KW trig & 4.2 & 0.044 & 36.8 & $<0.001$ \\
\hline
$\mathcal{SN}$ & 1 & KW trig & \textcolor{red}{0.0} & 0.355 & \textcolor{red}{0.0} & 0.907 \\
$\mathcal{SN}$ & 2 & KW trig & \textcolor{red}{0.9} & 0.227 & 27.0 & $<0.001$ \\
$\mathcal{SN}$ & 3 & KW trig & 8.3 & 0.006 & 60.6 & $<0.001$ \\
\hline
$\mathcal{T}$ & 1 & KW trig & 13.1 & 0.001 & 9.9 & 0.006 \\
$\mathcal{T}$ & 2 & KW trig & \textcolor{blue}{2.1} & 0.124 & 18.5 & $<0.001$ \\
$\mathcal{T}$ & 3 & KW trig & 6.4 & 0.014 & 42.3 & $<0.001$ \\
\hline
$\mathcal{ST}$ & 1 & KW trig & \textcolor{blue}{2.2} & 0.118 & 5.5 & 0.058 \\
$\mathcal{ST}$ & 2 & KW trig & \textcolor{blue}{3.8} & 0.053 & 33.2 & $<0.001$ \\
$\mathcal{ST}$ & 3 & KW trig & 11.0 & 0.001 & 66.5 & $<0.001$ \\

\hline

\noalign{\smallskip}
\end{tabular}
$$ 
\end{table}

==> tables/table_gbm_rest_100_900.tex <==
\begin{table}
\caption[]{Information criteria for the rest-frame hardness-duration distributions of 155 GRBs from the ``GBM all'' sample.
The durations were computed in the observer- and rest-frame energy windows $100-900$~keV, which in the latter case corresponds to the $\frac{100}{1+z}-\frac{900}{1+z}$~keV instrumental bandpass.
In both cases, the durations were corrected for the cosmological time dilation.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:rest_900keV}
$$ 
\begin{tabular}{llrrrr}
\hline
\noalign{\smallskip}

Statistics & Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & $w_i$ (BIC) \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

\multicolumn{6}{c}{In the $(100-900)/(1+z)$~keV energy window}  \\
\hline
$\mathcal{N}$ & 1 & 7.6 & 0.012 & \textcolor{red}{1.7} & 0.296\\
$\mathcal{N}$ & 2 & 6.4 & 0.021 & 18.7 & $<0.001$\\
$\mathcal{N}$ & 3 & 9.4 & 0.005 & 40.1 & $<0.001$\\
\hline
$\mathcal{SN}$ & 1 & 11.8 & 0.001 & 12.0 & 0.002\\
$\mathcal{SN}$ & 2 & 10.8 & 0.002 & 35.3 & $<0.001$\\
$\mathcal{SN}$ & 3 & 24.0 & $<0.001$ & 72.9 & $<0.001$\\
\hline
$\mathcal{T}$ & 1 & \textcolor{blue}{2.8} & 0.128 & \textcolor{red}{0.0} & 0.693\\
$\mathcal{T}$ & 2 & \textcolor{blue}{2.6} & 0.141 & 18.0 & $<0.001$\\
$\mathcal{T}$ & 3 & 5.8 & 0.029 & 39.4 & $<0.001$\\
\hline
$\mathcal{ST}$ & 1 & 5.5 & 0.033 & 8.7 & 0.009\\
$\mathcal{ST}$ & 2 & \textcolor{red}{0.0} & 0.518 & 27.6 & $<0.001$\\
$\mathcal{ST}$ & 3 & \textcolor{blue}{3.1} & 0.110 & 55.1 & $<0.001$\\
\hline

\multicolumn{6}{c}{In the $(100-900)$~keV energy window}\\
\hline
$\mathcal{N}$ & 1 & 15.0 & $<0.001$ & 3.1 & 0.070\\
$\mathcal{N}$ & 2 & 4.8 & 0.043 & 11.2 & 0.001\\
$\mathcal{N}$ & 3 & \textcolor{red}{0.0} & 0.470 & 24.6 & $<0.001$\\
\hline
$\mathcal{SN}$ & 1 & 5.8 & 0.026 & \textcolor{red}{0.0} & 0.330\\
$\mathcal{SN}$ & 2 & 9.8 & 0.003 & 28.3 & $<0.001$\\
$\mathcal{SN}$ & 3 & 11.1 & 0.002 & 54.0 & $<0.001$\\
\hline
$\mathcal{T}$ & 1 & 8.9 & 0.005 & \textcolor{red}{0.1} & 0.313\\
$\mathcal{T}$ & 2 & \textcolor{red}{0.7} & 0.331 & 10.1 & 0.002\\
$\mathcal{T}$ & 3 & 6.7 & 0.016 & 34.4 & $<0.001$\\
\hline
$\mathcal{ST}$ & 1 & \textcolor{blue}{3.1} & 0.100 & \textcolor{red}{0.3} & 0.284\\
$\mathcal{ST}$ & 2 & 9.8 & 0.003 & 31.4 & $<0.001$\\
$\mathcal{ST}$ & 3 & 13.7 & $<0.001$ & 59.6 & $<0.001$\\
\hline

\noalign{\smallskip}
\end{tabular}
$$ 
\end{table}

==> tables/table_obs.tex <==
\onecolumn
\begin{table}
\caption[]{Parameters of the fits with different models to the observer-frame hardness-duration distributions of the ``Total'' sample.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) \
        colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:obs_total}
$$
\begin{tabular}{llrrrrcccc}
\hline
\noalign{\smallskip}
Distr. &  Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & \
            $w_i$ (BIC) & $\mathcal{L}_\textrm{max}$ & $\mu$ & $\Sigma$ & $\lambda$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
$\mathcal{N}$ & 1 & 91.6 & $<0.001$ & 56.2 & $<0.001$ & -648.6 & (1.40, 2.23) & $\left( \begin{array}{cc}0.75 & -0.02 \\ -0.02 & 0.38 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 2 & 17.8 & $<0.001$ & 6.5 & 0.031 & -605.7 & (1.67, 2.23) & $\left( \begin{array}{cc}0.48 & 0.01 \\ 0.01 & 0.35 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -605.7 & (0.36, 2.21) & $\left( \begin{array}{cc}0.48 & -0.11 \\ 0.01 & 0.46 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 3 & \textcolor{red}{0.0} & 0.811 & 12.9 & 0.001 & -590.8 & (1.95, 2.16) & $\left( \begin{array}{cc}0.35 & 0.00 \\ 0.00 & 0.33 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -590.8 & (1.20, 2.23) & $\left( \begin{array}{cc}0.35 & 0.09 \\ 0.00 & 0.37 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -590.8 & (-0.42, 2.67) & $\left( \begin{array}{cc}0.35 & 0.10 \\ 0.00 & 0.39 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{SN}$ & 1 & 27.3 & $<0.001$ & \textcolor{red}{0.0} & 0.804 & -614.5 & (2.28, 2.15) & $\left( \begin{array}{cc}1.15 & -0.05 \\ -0.05 & 0.38 \end{array} \right)$ & (-3.82, 0.43) \\
\hline
$\mathcal{SN}$ & 2 & 16.0 & $<0.001$ & 20.8 & $<0.001$ & -600.8 & (1.27, 1.68) & $\left( \begin{array}{cc}0.93 & -0.27 \\ -0.27 & 0.57 \end{array} \right)$ & (-2.45, 2.89) \\
 &  &  &  &  &  & -600.8 & (1.59, 2.08) & $\left( \begin{array}{cc}0.93 & 0.02 \\ -0.27 & 0.39 \end{array} \right)$ & (0.54, 0.79) \\
\hline
$\mathcal{SN}$ & 3 & 12.0 & 0.002 & 48.9 & $<0.001$ & -590.8 & (1.79, 2.02) & $\left( \begin{array}{cc}0.39 & 0.03 \\ 0.03 & 0.37 \end{array} \right)$ & (0.51, 0.67) \\
 &  &  &  &  &  & -590.8 & (-0.24, 2.91) & $\left( \begin{array}{cc}0.39 & 0.15 \\ 0.03 & 0.42 \end{array} \right)$ & (-0.53, -0.68) \\
 &  &  &  &  &  & -590.8 & (1.49, 2.18) & $\left( \begin{array}{cc}0.39 & 0.07 \\ 0.03 & 0.38 \end{array} \right)$ & (-1.18, 0.38) \\
\hline
$\mathcal{T}$ & 1 & 81.8 & $<0.001$ & 50.5 & $<0.001$ & -642.7 & (1.47, 2.22) & $\left( \begin{array}{cc}0.66 & -0.00 \\ -0.00 & 0.35 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 2 & 21.4 & $<0.001$ & 14.2 & 0.001 & -606.5 & (1.68, 2.24) & $\left( \begin{array}{cc}0.47 & 0.00 \\ 0.00 & 0.35 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -606.5 & (0.40, 2.20) & $\left( \begin{array}{cc}0.47 & -0.12 \\ 0.00 & 0.45 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 3 & \textcolor{blue}{3.0} & 0.181 & 19.8 & $<0.001$ & -591.3 & (-0.42, 2.67) & $\left( \begin{array}{cc}0.38 & 0.10 \\ 0.10 & 0.39 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -591.3 & (1.23, 2.23) & $\left( \begin{array}{cc}0.38 & 0.09 \\ 0.10 & 0.36 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -591.3 & (1.99, 2.15) & $\left( \begin{array}{cc}0.38 & 0.00 \\ 0.10 & 0.32 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{ST}$ & 1 & 26.5 & $<0.001$ & 3.2 & 0.162 & -613.0 & (2.24, 2.17) & $\left( \begin{array}{cc}1.04 & -0.04 \\ -0.04 & 0.36 \end{array} \right)$ & (-3.19, 0.31) \\
\hline
$\mathcal{ST}$ & 2 & 18.6 & $<0.001$ & 27.4 & $<0.001$ & -601.1 & (1.60, 2.09) & $\left( \begin{array}{cc}0.47 & 0.01 \\ 0.01 & 0.38 \end{array} \right)$ & (0.37, 0.64) \\
 &  &  &  &  &  & -601.1 & (1.12, 1.66) & $\left( \begin{array}{cc}0.47 & -0.29 \\ 0.01 & 0.60 \end{array} \right)$ & (-2.58, 3.22) \\
\hline
$\mathcal{ST}$ & 3 & 9.8 & 0.006 & 50.8 & $<0.001$ & -588.7 & (-0.42, 3.03) & $\left( \begin{array}{cc}0.37 & 0.10 \\ 0.10 & 0.49 \end{array} \right)$ & (0.41, -2.07) \\
 &  &  &  &  &  & -588.7 & (1.63, 2.25) & $\left( \begin{array}{cc}0.37 & 0.08 \\ 0.10 & 0.37 \end{array} \right)$ & (-1.45, 0.15) \\
 &  &  &  &  &  & -588.7 & (1.93, 2.05) & $\left( \begin{array}{cc}0.37 & 0.02 \\ 0.10 & 0.34 \end{array} \right)$ & (0.30, 0.41) \\
\hline
\noalign{\smallskip}
\end{tabular}
$$
\end{table}
\twocolumn
\onecolumn
\begin{table}
\caption[]{Parameters of the fits with different models to the observer-frame hardness-duration distributions of the ``KW trig'' sample.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) \
        colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:obs_kw}
$$
\begin{tabular}{llrrrrcccc}
\hline
\noalign{\smallskip}
Distr. &  Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & \
            $w_i$ (BIC) & $\mathcal{L}_\textrm{max}$ & $\mu$ & $\Sigma$ & $\lambda$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
$\mathcal{N}$ & 1 & 58.8 & $<0.001$ & 33.4 & $<0.001$ & -286.5 & (1.27, 2.39) & $\left( \begin{array}{cc}0.76 & -0.01 \\ -0.01 & 0.34 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 2 & 13.6 & 0.001 & 7.8 & 0.014 & -257.9 & (1.51, 2.37) & $\left( \begin{array}{cc}0.49 & 0.03 \\ 0.03 & 0.30 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -257.9 & (-0.05, 2.51) & $\left( \begin{array}{cc}0.49 & -0.06 \\ 0.03 & 0.47 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 3 & \textcolor{red}{0.0} & 0.717 & 13.8 & 0.001 & -245.1 & (1.79, 2.29) & $\left( \begin{array}{cc}0.35 & 0.05 \\ 0.05 & 0.26 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -245.1 & (1.06, 2.42) & $\left( \begin{array}{cc}0.35 & 0.14 \\ 0.05 & 0.32 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -245.1 & (-0.44, 2.82) & $\left( \begin{array}{cc}0.35 & 0.15 \\ 0.05 & 0.31 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{SN}$ & 1 & 18.9 & $<0.001$ & \textcolor{red}{0.0} & 0.710 & -264.5 & (2.15, 2.27) & $\left( \begin{array}{cc}1.15 & -0.08 \\ -0.08 & 0.35 \end{array} \right)$ & (-5.00, 1.15) \\
\hline
$\mathcal{SN}$ & 2 & 23.0 & $<0.001$ & 30.2 & $<0.001$ & -258.6 & (1.26, 1.94) & $\left( \begin{array}{cc}0.98 & -0.24 \\ -0.24 & 0.52 \end{array} \right)$ & (-2.17, 2.07) \\
 &  &  &  &  &  & -258.6 & (1.46, 2.22) & $\left( \begin{array}{cc}0.98 & 0.05 \\ -0.24 & 0.35 \end{array} \right)$ & (0.67, 0.94) \\
\hline
$\mathcal{SN}$ & 3 & 10.1 & 0.005 & 43.5 & $<0.001$ & -244.2 & (-0.14, 2.86) & $\left( \begin{array}{cc}0.51 & 0.15 \\ 0.15 & 0.31 \end{array} \right)$ & (-1.68, 0.45) \\
 &  &  &  &  &  & -244.2 & (1.69, 2.53) & $\left( \begin{array}{cc}0.51 & 0.15 \\ 0.15 & 0.33 \end{array} \right)$ & (-2.29, -0.68) \\
 &  &  &  &  &  & -244.2 & (1.82, 2.09) & $\left( \begin{array}{cc}0.51 & 0.11 \\ 0.15 & 0.37 \end{array} \right)$ & (0.88, 1.27) \\
\hline
$\mathcal{T}$ & 1 & 50.7 & $<0.001$ & 28.5 & $<0.001$ & -281.4 & (1.36, 2.38) & $\left( \begin{array}{cc}0.64 & -0.00 \\ -0.00 & 0.30 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 2 & 16.2 & $<0.001$ & 13.7 & 0.001 & -258.2 & (-0.06, 2.52) & $\left( \begin{array}{cc}0.59 & -0.06 \\ -0.06 & 0.47 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -258.2 & (1.51, 2.37) & $\left( \begin{array}{cc}0.59 & 0.03 \\ -0.06 & 0.30 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 3 & \textcolor{red}{1.9} & 0.277 & 18.9 & $<0.001$ & -245.0 & (1.12, 2.40) & $\left( \begin{array}{cc}0.49 & 0.12 \\ 0.12 & 0.31 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -245.0 & (-0.44, 2.82) & $\left( \begin{array}{cc}0.49 & 0.15 \\ 0.12 & 0.30 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -245.0 & (1.85, 2.28) & $\left( \begin{array}{cc}0.49 & 0.05 \\ 0.12 & 0.25 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{ST}$ & 1 & 17.5 & $<0.001$ & \textcolor{red}{1.9} & 0.274 & -262.9 & (2.10, 2.29) & $\left( \begin{array}{cc}0.99 & -0.06 \\ -0.06 & 0.32 \end{array} \right)$ & (-3.73, 0.80) \\
\hline
$\mathcal{ST}$ & 2 & 25.5 & $<0.001$ & 36.0 & $<0.001$ & -258.9 & (1.22, 1.96) & $\left( \begin{array}{cc}0.97 & -0.23 \\ -0.23 & 0.51 \end{array} \right)$ & (-2.09, 1.90) \\
 &  &  &  &  &  & -258.9 & (1.47, 2.24) & $\left( \begin{array}{cc}0.97 & 0.04 \\ -0.23 & 0.34 \end{array} \right)$ & (0.58, 0.82) \\
\hline
$\mathcal{ST}$ & 3 & 19.5 & $<0.001$ & 56.1 & $<0.001$ & -247.9 & (1.57, 2.29) & $\left( \begin{array}{cc}0.40 & 0.02 \\ 0.02 & 0.32 \end{array} \right)$ & (1.05, 1.20) \\
 &  &  &  &  &  & -247.9 & (-0.29, 3.01) & $\left( \begin{array}{cc}0.40 & 0.18 \\ 0.02 & 0.34 \end{array} \right)$ & (-0.32, -0.64) \\
 &  &  &  &  &  & -247.9 & (1.33, 2.34) & $\left( \begin{array}{cc}0.40 & 0.06 \\ 0.02 & 0.32 \end{array} \right)$ & (-1.42, -0.89) \\
\hline
\noalign{\smallskip}
\end{tabular}
$$
\end{table}
\twocolumn
\onecolumn
\begin{table}
\caption[]{Parameters of the fits with different models to the observer-frame hardness-duration distributions of the ``KW \& BAT'' sample.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) \
        colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:obs_bat}
$$
\begin{tabular}{llrrrrcccc}
\hline
\noalign{\smallskip}
Distr. &  Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & \
            $w_i$ (BIC) & $\mathcal{L}_\textrm{max}$ & $\mu$ & $\Sigma$ & $\lambda$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
$\mathcal{N}$ & 1 & 13.6 & 0.001 & 7.4 & 0.023 & -196.7 & (1.63, 2.04) & $\left( \begin{array}{cc}0.62 & 0.05 \\ 0.05 & 0.31 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 2 & 7.9 & 0.012 & 20.4 & $<0.001$ & -187.9 & (1.30, 2.03) & $\left( \begin{array}{cc}0.55 & 0.07 \\ 0.07 & 0.31 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -187.9 & (2.14, 2.06) & $\left( \begin{array}{cc}0.55 & 0.03 \\ 0.07 & 0.31 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 3 & 4.4 & 0.067 & 35.6 & $<0.001$ & -180.1 & (1.94, 1.68) & $\left( \begin{array}{cc}0.40 & 0.03 \\ 0.03 & 0.10 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -180.1 & (2.23, 2.21) & $\left( \begin{array}{cc}0.40 & 0.00 \\ 0.03 & 0.23 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -180.1 & (1.32, 2.07) & $\left( \begin{array}{cc}0.40 & 0.09 \\ 0.03 & 0.29 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{SN}$ & 1 & \textcolor{red}{0.0} & 0.609 & \textcolor{red}{0.0} & 0.932 & -188.0 & (2.40, 2.17) & $\left( \begin{array}{cc}0.98 & 0.11 \\ 0.11 & 0.32 \end{array} \right)$ & (-3.95, -0.67) \\
\hline
$\mathcal{SN}$ & 2 & 13.1 & 0.001 & 38.1 & $<0.001$ & -186.5 & (1.67, 2.01) & $\left( \begin{array}{cc}0.67 & 0.06 \\ 0.06 & 0.32 \end{array} \right)$ & (-1.80, 0.80) \\
 &  &  &  &  &  & -186.5 & (1.99, 2.12) & $\left( \begin{array}{cc}0.67 & 0.02 \\ 0.06 & 0.32 \end{array} \right)$ & (1.07, -0.72) \\
\hline
$\mathcal{SN}$ & 3 & 5.0 & 0.050 & 54.9 & $<0.001$ & -174.4 & (1.36, 2.09) & $\left( \begin{array}{cc}0.32 & -0.02 \\ -0.02 & 0.26 \end{array} \right)$ & (0.60, 0.84) \\
 &  &  &  &  &  & -174.4 & (2.18, 2.43) & $\left( \begin{array}{cc}0.32 & -0.02 \\ -0.02 & 0.32 \end{array} \right)$ & (0.15, -1.24) \\
 &  &  &  &  &  & -174.4 & (1.67, 1.55) & $\left( \begin{array}{cc}0.32 & -0.10 \\ -0.02 & 0.26 \end{array} \right)$ & (-2.32, 3.66) \\
\hline
$\mathcal{T}$ & 1 & 16.3 & $<0.001$ & 13.2 & 0.001 & -197.1 & (1.64, 2.04) & $\left( \begin{array}{cc}0.61 & 0.05 \\ 0.05 & 0.31 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 2 & 10.2 & 0.004 & 25.9 & $<0.001$ & -188.1 & (2.14, 2.06) & $\left( \begin{array}{cc}0.28 & 0.03 \\ 0.03 & 0.31 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -188.1 & (1.30, 2.04) & $\left( \begin{array}{cc}0.28 & 0.08 \\ 0.03 & 0.31 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 3 & \textcolor{blue}{3.5} & 0.106 & 37.8 & $<0.001$ & -178.7 & (2.19, 2.20) & $\left( \begin{array}{cc}0.24 & -0.00 \\ -0.00 & 0.27 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -178.7 & (1.24, 1.75) & $\left( \begin{array}{cc}0.24 & -0.02 \\ -0.00 & 0.17 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -178.7 & (1.43, 2.22) & $\left( \begin{array}{cc}0.24 & -0.03 \\ -0.00 & 0.23 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{ST}$ & 1 & \textcolor{blue}{3.0} & 0.136 & 6.1 & 0.044 & -188.4 & (2.40, 2.17) & $\left( \begin{array}{cc}0.97 & 0.11 \\ 0.11 & 0.32 \end{array} \right)$ & (-3.87, -0.66) \\
\hline
$\mathcal{ST}$ & 2 & 15.8 & $<0.001$ & 43.9 & $<0.001$ & -186.8 & (1.66, 2.01) & $\left( \begin{array}{cc}0.65 & 0.06 \\ 0.06 & 0.32 \end{array} \right)$ & (-1.63, 0.75) \\
 &  &  &  &  &  & -186.8 & (2.00, 2.12) & $\left( \begin{array}{cc}0.65 & 0.02 \\ 0.06 & 0.31 \end{array} \right)$ & (0.95, -0.65) \\
\hline
$\mathcal{ST}$ & 3 & 7.5 & 0.014 & 60.5 & $<0.001$ & -174.7 & (1.38, 2.08) & $\left( \begin{array}{cc}0.29 & -0.02 \\ -0.02 & 0.26 \end{array} \right)$ & (0.48, 0.96) \\
 &  &  &  &  &  & -174.7 & (2.17, 2.42) & $\left( \begin{array}{cc}0.29 & -0.01 \\ -0.02 & 0.31 \end{array} \right)$ & (0.10, -1.18) \\
 &  &  &  &  &  & -174.7 & (1.66, 1.55) & $\left( \begin{array}{cc}0.29 & -0.10 \\ -0.02 & 0.26 \end{array} \right)$ & (-2.19, 3.57) \\
\hline
\noalign{\smallskip}
\end{tabular}
$$
\end{table}
\twocolumn
\onecolumn
\begin{table}
\caption[]{Parameters of the fits with different models to the observer-frame hardness-duration distributions of the ``GBM all'' sample.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) \
        colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:obs_gbm}
$$
\begin{tabular}{llrrrrcccc}
\hline
\noalign{\smallskip}
Distr. &  Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & \
            $w_i$ (BIC) & $\mathcal{L}_\textrm{max}$ & $\mu$ & $\Sigma$ & $\lambda$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
$\mathcal{N}$ & 1 & 57.1 & $<0.001$ & 40.1 & $<0.001$ & -300.0 & (1.37, 2.28) & $\left( \begin{array}{cc}0.75 & 0.01 \\ 0.01 & 0.47 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 2 & 11.2 & 0.001 & 12.9 & 0.002 & -271.0 & (1.59, 2.26) & $\left( \begin{array}{cc}0.46 & 0.05 \\ 0.05 & 0.45 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -271.0 & (-0.14, 2.43) & $\left( \begin{array}{cc}0.46 & 0.02 \\ 0.05 & 0.53 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 3 & \textcolor{red}{0.0} & 0.395 & 20.4 & $<0.001$ & -259.4 & (1.50, 2.23) & $\left( \begin{array}{cc}0.45 & 0.05 \\ 0.05 & 0.36 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -259.4 & (-0.21, 2.46) & $\left( \begin{array}{cc}0.45 & 0.04 \\ 0.05 & 0.54 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -259.4 & (2.09, 2.45) & $\left( \begin{array}{cc}0.45 & 0.01 \\ 0.05 & 0.83 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{SN}$ & 1 & 24.4 & $<0.001$ & 13.5 & 0.001 & -281.6 & (2.19, 2.23) & $\left( \begin{array}{cc}1.11 & -0.02 \\ -0.02 & 0.47 \end{array} \right)$ & (-3.79, 0.42) \\
\hline
$\mathcal{SN}$ & 2 & 8.1 & 0.007 & 22.3 & $<0.001$ & -265.5 & (1.41, 1.83) & $\left( \begin{array}{cc}0.48 & 0.11 \\ 0.11 & 0.62 \end{array} \right)$ & (0.62, 1.87) \\
 &  &  &  &  &  & -265.5 & (-0.10, 2.05) & $\left( \begin{array}{cc}0.48 & -0.00 \\ 0.11 & 0.65 \end{array} \right)$ & (-0.09, 1.01) \\
\hline
$\mathcal{SN}$ & 3 & 9.1 & 0.004 & 48.3 & $<0.001$ & -258.0 & (1.79, 2.33) & $\left( \begin{array}{cc}0.68 & 0.11 \\ 0.11 & 0.35 \end{array} \right)$ & (-1.90, -0.88) \\
 &  &  &  &  &  & -258.0 & (1.72, 1.92) & $\left( \begin{array}{cc}0.68 & 0.09 \\ 0.11 & 0.78 \end{array} \right)$ & (1.25, 2.10) \\
 &  &  &  &  &  & -258.0 & (-0.41, 2.50) & $\left( \begin{array}{cc}0.68 & 0.17 \\ 0.11 & 0.51 \end{array} \right)$ & (-0.19, 0.41) \\
\hline
$\mathcal{T}$ & 1 & 26.4 & $<0.001$ & 12.5 & 0.002 & -283.6 & (1.48, 2.25) & $\left( \begin{array}{cc}0.55 & 0.02 \\ 0.02 & 0.35 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 2 & \textcolor{red}{1.9} & 0.153 & 6.7 & 0.034 & -265.3 & (-0.20, 2.44) & $\left( \begin{array}{cc}0.48 & -0.02 \\ -0.02 & 0.45 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -265.3 & (1.57, 2.25) & $\left( \begin{array}{cc}0.48 & 0.04 \\ -0.02 & 0.37 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 3 & \textcolor{red}{2.0} & 0.145 & 25.5 & $<0.001$ & -259.4 & (2.08, 2.42) & $\left( \begin{array}{cc}0.20 & 0.01 \\ 0.01 & 0.77 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -259.4 & (-0.23, 2.47) & $\left( \begin{array}{cc}0.20 & 0.04 \\ 0.01 & 0.52 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -259.4 & (1.50, 2.23) & $\left( \begin{array}{cc}0.20 & 0.05 \\ 0.01 & 0.35 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{ST}$ & 1 & 7.7 & 0.008 & \textcolor{red}{0.0} & 0.962 & -272.2 & (2.00, 2.18) & $\left( \begin{array}{cc}0.76 & -0.02 \\ -0.02 & 0.37 \end{array} \right)$ & (-2.06, 0.47) \\
\hline
$\mathcal{ST}$ & 2 & 7.6 & 0.009 & 24.9 & $<0.001$ & -264.2 & (1.43, 1.96) & $\left( \begin{array}{cc}0.45 & 0.08 \\ 0.08 & 0.47 \end{array} \right)$ & (0.42, 1.09) \\
 &  &  &  &  &  & -264.2 & (-0.08, 2.16) & $\left( \begin{array}{cc}0.45 & -0.04 \\ 0.08 & 0.53 \end{array} \right)$ & (-0.20, 0.68) \\
\hline
$\mathcal{ST}$ & 3 & \textcolor{red}{0.7} & 0.278 & 43.0 & $<0.001$ & -252.8 & (1.80, 2.25) & $\left( \begin{array}{cc}0.60 & 0.05 \\ 0.05 & 0.32 \end{array} \right)$ & (-2.24, 0.01) \\
 &  &  &  &  &  & -252.8 & (2.03, 1.87) & $\left( \begin{array}{cc}0.60 & 0.04 \\ 0.05 & 0.68 \end{array} \right)$ & (0.40, 1.46) \\
 &  &  &  &  &  & -252.8 & (-0.74, 2.65) & $\left( \begin{array}{cc}0.60 & 0.12 \\ 0.05 & 0.41 \end{array} \right)$ & (13.15, -3.73) \\
\hline
\noalign{\smallskip}
\end{tabular}
$$
\end{table}
\twocolumn



==> tables/table_obsT90.tex <==
\begin{table}
\caption[]{Information criteria for the rest-frame hardness-observer-frame duration distributions.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:obsT90}
$$ 
\begin{tabular}{llrrrrr}
\hline
\noalign{\smallskip}
Statistics & Cl. & Sample & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & $w_i$ (BIC) \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

$\mathcal{N}$ & 1 & Total & 66.7 & $<0.001$ & 56.2 & $<0.001$ \\
$\mathcal{N}$ & 2 & Total & \textcolor{red}{0.6} & 0.179 & 14.2 & 0.001 \\
$\mathcal{N}$ & 3 & Total & \textcolor{red}{0.7} & 0.170 & 38.3 & $<0.001$ \\
\hline
$\mathcal{SN}$ & 1 & Total & \textcolor{blue}{2.5} & 0.069 & \textcolor{red}{0.0} & 0.950 \\
$\mathcal{SN}$ & 2 & Total & 5.2 & 0.018 & 34.8 & $<0.001$ \\
$\mathcal{SN}$ & 3 & Total & \textcolor{red}{0.0} & 0.241 & 61.7 & $<0.001$ \\
\hline
$\mathcal{T}$ & 1 & Total & 61.3 & $<0.001$ & 54.8 & $<0.001$ \\
$\mathcal{T}$ & 2 & Total & \textcolor{blue}{4.0} & 0.033 & 21.6 & $<0.001$ \\
$\mathcal{T}$ & 3 & Total & \textcolor{blue}{2.4} & 0.073 & 44.1 & $<0.001$ \\
\hline
$\mathcal{ST}$ & 1 & Total & 4.4 & 0.027 & 5.9 & 0.050 \\
$\mathcal{ST}$ & 2 & Total & 8.9 & 0.003 & 42.5 & $<0.001$ \\
$\mathcal{ST}$ & 3 & Total & \textcolor{red}{0.5} & 0.188 & 66.2 & $<0.001$ \\
\hline

\noalign{\smallskip}
\end{tabular}
$$ 
\end{table}

==> tables/table_rest.tex <==
\onecolumn
\begin{table}
\caption[]{Parameters of the fits with different models to the rest-frame hardness-duration distributions of the ``Total'' sample.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue \
        ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:rest_total}
$$
\begin{tabular}{llrrrrcccc}
\hline
\noalign{\smallskip}
Distr. &  Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & \
            $w_i$ (BIC) & $\mathcal{L}_\textrm{max}$ & $\mu$ & $\Sigma$ & $\lambda$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
$\mathcal{N}$ & 1 & 45.8 & $<0.001$ & 37.7 & $<0.001$ & -659.3 & (0.99, 2.64) & $\left( \begin{array}{cc}0.73 & -0.01 \\ -0.01 & 0.40 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 2 & 5.5 & 0.044 & 21.5 & $<0.001$ & -633.1 & (0.34, 2.55) & $\left( \begin{array}{cc}0.71 & -0.06 \\ -0.06 & 0.43 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -633.1 & (1.34, 2.70) & $\left( \begin{array}{cc}0.71 & -0.03 \\ -0.06 & 0.37 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 3 & 7.1 & 0.020 & 47.3 & $<0.001$ & -628.0 & (1.37, 2.34) & $\left( \begin{array}{cc}0.49 & -0.02 \\ -0.02 & 0.25 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -628.0 & (0.19, 2.56) & $\left( \begin{array}{cc}0.49 & -0.07 \\ -0.02 & 0.45 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -628.0 & (1.25, 2.90) & $\left( \begin{array}{cc}0.49 & 0.01 \\ -0.02 & 0.25 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{SN}$ & 1 & \textcolor{red}{0.0} & 0.696 & \textcolor{red}{0.0} & 0.959 & -634.4 & (1.83, 2.70) & $\left( \begin{array}{cc}1.11 & 0.02 \\ 0.02 & 0.41 \end{array} \right)$ & (-3.35, -0.38) \\
\hline
$\mathcal{SN}$ & 2 & 9.3 & 0.007 & 41.4 & $<0.001$ & -631.1 & (0.81, 2.71) & $\left( \begin{array}{cc}0.82 & -0.00 \\ -0.00 & 0.46 \end{array} \right)$ & (-1.17, -0.71) \\
 &  &  &  &  &  & -631.1 & (1.11, 2.97) & $\left( \begin{array}{cc}0.82 & -0.10 \\ -0.00 & 0.45 \end{array} \right)$ & (0.91, -1.14) \\
\hline
$\mathcal{SN}$ & 3 & 16.3 & $<0.001$ & 80.6 & $<0.001$ & -626.6 & (1.31, 2.96) & $\left( \begin{array}{cc}0.40 & -0.10 \\ -0.10 & 0.48 \end{array} \right)$ & (0.93, -1.27) \\
 &  &  &  &  &  & -626.6 & (1.02, 2.84) & $\left( \begin{array}{cc}0.40 & 0.11 \\ -0.10 & 0.45 \end{array} \right)$ & (-1.12, -0.95) \\
 &  &  &  &  &  & -626.6 & (0.04, 2.94) & $\left( \begin{array}{cc}0.40 & 0.05 \\ -0.10 & 0.48 \end{array} \right)$ & (-0.81, -0.65) \\
\hline
$\mathcal{T}$ & 1 & 46.4 & $<0.001$ & 42.4 & $<0.001$ & -658.6 & (1.01, 2.65) & $\left( \begin{array}{cc}0.70 & -0.01 \\ -0.01 & 0.39 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 2 & 8.4 & 0.010 & 28.5 & $<0.001$ & -633.6 & (1.33, 2.69) & $\left( \begin{array}{cc}0.45 & -0.03 \\ -0.03 & 0.37 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -633.6 & (0.30, 2.55) & $\left( \begin{array}{cc}0.45 & -0.07 \\ -0.03 & 0.43 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 3 & 13.2 & 0.001 & 57.4 & $<0.001$ & -630.0 & (0.04, 2.59) & $\left( \begin{array}{cc}0.64 & -0.06 \\ -0.06 & 0.46 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -630.0 & (0.94, 2.67) & $\left( \begin{array}{cc}0.64 & 0.01 \\ -0.06 & 0.36 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -630.0 & (1.61, 2.65) & $\left( \begin{array}{cc}0.64 & -0.04 \\ -0.06 & 0.39 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{ST}$ & 1 & \textcolor{blue}{2.3} & 0.220 & 6.3 & 0.041 & -634.6 & (1.81, 2.70) & $\left( \begin{array}{cc}1.06 & 0.02 \\ 0.02 & 0.40 \end{array} \right)$ & (-3.14, -0.37) \\
\hline
$\mathcal{ST}$ & 2 & 12.7 & 0.001 & 48.8 & $<0.001$ & -631.7 & (0.74, 2.68) & $\left( \begin{array}{cc}0.79 & -0.01 \\ -0.01 & 0.45 \end{array} \right)$ & (-1.09, -0.60) \\
 &  &  &  &  &  & -631.7 & (1.12, 2.95) & $\left( \begin{array}{cc}0.79 & -0.09 \\ -0.01 & 0.44 \end{array} \right)$ & (0.81, -1.02) \\
\hline
$\mathcal{ST}$ & 3 & 16.7 & $<0.001$ & 84.9 & $<0.001$ & -625.8 & (1.06, 2.84) & $\left( \begin{array}{cc}0.55 & 0.11 \\ 0.11 & 0.45 \end{array} \right)$ & (-1.11, -0.88) \\
 &  &  &  &  &  & -625.8 & (-0.40, 3.13) & $\left( \begin{array}{cc}0.55 & 0.09 \\ 0.11 & 0.45 \end{array} \right)$ & (-0.34, -0.89) \\
 &  &  &  &  &  & -625.8 & (1.35, 2.93) & $\left( \begin{array}{cc}0.55 & -0.09 \\ 0.11 & 0.47 \end{array} \right)$ & (0.88, -1.14) \\
\hline
\noalign{\smallskip}
\end{tabular}
$$
\end{table}
\twocolumn
\onecolumn
\begin{table}
\caption[]{Parameters of the fits with different models to the rest-frame hardness-duration distributions of the ``KW trig'' sample.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue \
        ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:rest_kw}
$$
\begin{tabular}{llrrrrcccc}
\hline
\noalign{\smallskip}
Distr. &  Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & \
            $w_i$ (BIC) & $\mathcal{L}_\textrm{max}$ & $\mu$ & $\Sigma$ & $\lambda$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
$\mathcal{N}$ & 1 & 23.3 & $<0.001$ & 16.8 & $<0.001$ & -298.5 & (0.91, 2.75) & $\left( \begin{array}{cc}0.74 & -0.01 \\ -0.01 & 0.37 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 2 & \textcolor{blue}{2.4} & 0.155 & 15.5 & $<0.001$ & -282.0 & (0.38, 2.62) & $\left( \begin{array}{cc}0.78 & -0.11 \\ -0.11 & 0.43 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -282.0 & (1.25, 2.84) & $\left( \begin{array}{cc}0.78 & -0.01 \\ -0.11 & 0.29 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 3 & 14.3 & $<0.001$ & 46.9 & $<0.001$ & -282.0 & (-0.24, 2.83) & $\left( \begin{array}{cc}0.56 & -0.01 \\ -0.01 & 0.43 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -282.0 & (1.50, 2.71) & $\left( \begin{array}{cc}0.56 & 0.01 \\ -0.01 & 0.36 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -282.0 & (0.78, 2.77) & $\left( \begin{array}{cc}0.56 & 0.05 \\ -0.01 & 0.34 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{SN}$ & 1 & \textcolor{red}{0.0} & 0.514 & \textcolor{red}{0.0} & 0.916 & -284.8 & (1.79, 2.73) & $\left( \begin{array}{cc}1.14 & -0.02 \\ -0.02 & 0.37 \end{array} \right)$ & (-3.78, 0.12) \\
\hline
$\mathcal{SN}$ & 2 & 5.6 & 0.031 & 31.8 & $<0.001$ & -279.7 & (1.11, 3.12) & $\left( \begin{array}{cc}0.47 & -0.06 \\ -0.06 & 0.48 \end{array} \right)$ & (0.59, -2.21) \\
 &  &  &  &  &  & -279.7 & (0.59, 2.77) & $\left( \begin{array}{cc}0.47 & -0.04 \\ -0.06 & 0.45 \end{array} \right)$ & (-1.60, -0.45) \\
\hline
$\mathcal{SN}$ & 3 & 10.9 & 0.002 & 63.2 & $<0.001$ & -274.3 & (-0.33, 3.00) & $\left( \begin{array}{cc}0.50 & 0.08 \\ 0.08 & 0.37 \end{array} \right)$ & (-0.70, 0.15) \\
 &  &  &  &  &  & -274.3 & (1.48, 3.01) & $\left( \begin{array}{cc}0.50 & -0.00 \\ 0.08 & 0.51 \end{array} \right)$ & (1.11, -3.46) \\
 &  &  &  &  &  & -274.3 & (1.04, 3.18) & $\left( \begin{array}{cc}0.50 & 0.16 \\ 0.08 & 0.52 \end{array} \right)$ & (-1.06, -2.86) \\
\hline
$\mathcal{T}$ & 1 & 23.3 & $<0.001$ & 20.0 & $<0.001$ & -297.5 & (0.95, 2.76) & $\left( \begin{array}{cc}0.68 & -0.01 \\ -0.01 & 0.34 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 2 & 4.8 & 0.047 & 21.2 & $<0.001$ & -282.3 & (1.25, 2.83) & $\left( \begin{array}{cc}0.44 & -0.01 \\ -0.01 & 0.28 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -282.3 & (0.37, 2.62) & $\left( \begin{array}{cc}0.44 & -0.11 \\ -0.01 & 0.43 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 3 & 16.3 & $<0.001$ & 52.2 & $<0.001$ & -282.0 & (1.51, 2.71) & $\left( \begin{array}{cc}0.32 & 0.01 \\ 0.01 & 0.36 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -282.0 & (-0.28, 2.84) & $\left( \begin{array}{cc}0.32 & -0.00 \\ 0.01 & 0.43 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -282.0 & (0.78, 2.77) & $\left( \begin{array}{cc}0.32 & 0.05 \\ 0.01 & 0.34 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{ST}$ & 1 & \textcolor{red}{1.5} & 0.243 & 4.8 & 0.083 & -284.6 & (1.74, 2.76) & $\left( \begin{array}{cc}1.04 & -0.00 \\ -0.00 & 0.35 \end{array} \right)$ & (-3.28, -0.08) \\
\hline
$\mathcal{ST}$ & 2 & 8.5 & 0.007 & 37.9 & $<0.001$ & -280.1 & (0.79, 2.73) & $\left( \begin{array}{cc}0.89 & -0.05 \\ -0.05 & 0.44 \end{array} \right)$ & (-1.44, -0.53) \\
 &  &  &  &  &  & -280.1 & (1.14, 3.11) & $\left( \begin{array}{cc}0.89 & -0.06 \\ -0.05 & 0.43 \end{array} \right)$ & (0.56, -1.83) \\
\hline
$\mathcal{ST}$ & 3 & 24.5 & $<0.001$ & 80.0 & $<0.001$ & -280.1 & (1.01, 2.80) & $\left( \begin{array}{cc}0.49 & 0.04 \\ 0.04 & 0.25 \end{array} \right)$ & (0.90, 0.93) \\
 &  &  &  &  &  & -280.1 & (0.52, 2.55) & $\left( \begin{array}{cc}0.49 & -0.10 \\ 0.04 & 0.44 \end{array} \right)$ & (-1.05, 0.70) \\
 &  &  &  &  &  & -280.1 & (1.05, 2.58) & $\left( \begin{array}{cc}0.49 & -0.05 \\ 0.04 & 0.34 \end{array} \right)$ & (0.66, -1.16) \\
\hline
\noalign{\smallskip}
\end{tabular}
$$
\end{table}
\twocolumn
\onecolumn
\begin{table}
\caption[]{Parameters of the fits with different models to the rest-frame hardness-duration distributions of the ``KW \& BAT'' sample.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue \
        ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:rest_bat}
$$
\begin{tabular}{llrrrrcccc}
\hline
\noalign{\smallskip}
Distr. &  Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & \
            $w_i$ (BIC) & $\mathcal{L}_\textrm{max}$ & $\mu$ & $\Sigma$ & $\lambda$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
$\mathcal{N}$ & 1 & \textcolor{red}{1.6} & 0.149 & \textcolor{red}{0.0} & 0.946 & -235.6 & (1.14, 2.54) & $\left( \begin{array}{cc}0.63 & 0.02 \\ 0.02 & 0.38 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 2 & \textcolor{red}{0.0} & 0.331 & 17.1 & $<0.001$ & -228.7 & (1.47, 2.60) & $\left( \begin{array}{cc}0.41 & -0.04 \\ -0.04 & 0.37 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -228.7 & (0.56, 2.45) & $\left( \begin{array}{cc}0.41 & 0.03 \\ -0.04 & 0.38 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 3 & \textcolor{red}{0.3} & 0.285 & 36.1 & $<0.001$ & -222.9 & (0.46, 2.27) & $\left( \begin{array}{cc}0.50 & -0.03 \\ -0.03 & 0.29 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -222.9 & (1.11, 2.56) & $\left( \begin{array}{cc}0.50 & -0.13 \\ -0.03 & 0.32 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -222.9 & (1.72, 2.74) & $\left( \begin{array}{cc}0.50 & -0.11 \\ -0.03 & 0.35 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{SN}$ & 1 & 6.5 & 0.013 & 11.1 & 0.004 & -236.0 & (1.48, 2.34) & $\left( \begin{array}{cc}0.72 & -0.04 \\ -0.04 & 0.43 \end{array} \right)$ & (-0.88, 0.82) \\
\hline
$\mathcal{SN}$ & 2 & 6.3 & 0.014 & 35.9 & $<0.001$ & -227.9 & (0.88, 2.27) & $\left( \begin{array}{cc}0.60 & -0.03 \\ -0.03 & 0.42 \end{array} \right)$ & (-1.67, 1.17) \\
 &  &  &  &  &  & -227.9 & (1.35, 2.39) & $\left( \begin{array}{cc}0.60 & -0.01 \\ -0.03 & 0.43 \end{array} \right)$ & (0.46, 0.83) \\
\hline
$\mathcal{SN}$ & 3 & 8.2 & 0.005 & 62.8 & $<0.001$ & -220.9 & (1.59, 2.59) & $\left( \begin{array}{cc}0.32 & -0.08 \\ -0.08 & 0.38 \end{array} \right)$ & (0.66, 0.69) \\
 &  &  &  &  &  & -220.9 & (1.25, 2.60) & $\left( \begin{array}{cc}0.32 & -0.09 \\ -0.08 & 0.35 \end{array} \right)$ & (-1.88, -1.13) \\
 &  &  &  &  &  & -220.9 & (0.68, 2.03) & $\left( \begin{array}{cc}0.32 & -0.12 \\ -0.08 & 0.33 \end{array} \right)$ & (-2.79, 1.93) \\
\hline
$\mathcal{T}$ & 1 & 4.4 & 0.037 & 5.9 & 0.050 & -236.0 & (1.14, 2.54) & $\left( \begin{array}{cc}0.62 & 0.02 \\ 0.02 & 0.38 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 2 & \textcolor{blue}{2.8} & 0.082 & 23.0 & $<0.001$ & -229.2 & (0.60, 2.47) & $\left( \begin{array}{cc}0.51 & 0.04 \\ 0.04 & 0.38 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -229.2 & (1.49, 2.59) & $\left( \begin{array}{cc}0.51 & -0.04 \\ 0.04 & 0.37 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 3 & \textcolor{blue}{2.9} & 0.078 & 41.9 & $<0.001$ & -223.2 & (1.71, 2.72) & $\left( \begin{array}{cc}0.29 & -0.10 \\ -0.10 & 0.35 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -223.2 & (1.09, 2.55) & $\left( \begin{array}{cc}0.29 & -0.13 \\ -0.10 & 0.32 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -223.2 & (0.40, 2.27) & $\left( \begin{array}{cc}0.29 & -0.03 \\ -0.10 & 0.29 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{ST}$ & 1 & 8.8 & 0.004 & 16.5 & $<0.001$ & -236.1 & (1.46, 2.36) & $\left( \begin{array}{cc}0.70 & -0.03 \\ -0.03 & 0.42 \end{array} \right)$ & (-0.80, 0.71) \\
\hline
$\mathcal{ST}$ & 2 & 9.4 & 0.003 & 42.1 & $<0.001$ & -228.4 & (0.86, 2.27) & $\left( \begin{array}{cc}0.58 & -0.02 \\ -0.02 & 0.42 \end{array} \right)$ & (-1.47, 1.06) \\
 &  &  &  &  &  & -228.4 & (1.35, 2.41) & $\left( \begin{array}{cc}0.58 & -0.01 \\ -0.02 & 0.42 \end{array} \right)$ & (0.44, 0.75) \\
\hline
$\mathcal{ST}$ & 3 & 12.5 & 0.001 & 70.1 & $<0.001$ & -222.0 & (1.26, 2.75) & $\left( \begin{array}{cc}0.45 & -0.01 \\ -0.01 & 0.29 \end{array} \right)$ & (0.24, 0.27) \\
 &  &  &  &  &  & -222.0 & (1.65, 2.05) & $\left( \begin{array}{cc}0.45 & -0.04 \\ -0.01 & 0.25 \end{array} \right)$ & (-0.67, 1.54) \\
 &  &  &  &  &  & -222.0 & (0.77, 2.14) & $\left( \begin{array}{cc}0.45 & -0.07 \\ -0.01 & 0.41 \end{array} \right)$ & (-3.18, 2.62) \\
\hline
\noalign{\smallskip}
\end{tabular}
$$
\end{table}
\twocolumn
\onecolumn
\begin{table}
\caption[]{Parameters of the fits with different models to the rest-frame hardness-duration distributions of the ``GBM all'' sample.
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue \
        ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:rest_gbm}
$$
\begin{tabular}{llrrrrcccc}
\hline
\noalign{\smallskip}
Distr. &  Cl. & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & \
            $w_i$ (BIC) & $\mathcal{L}_\textrm{max}$ & $\mu$ & $\Sigma$ & $\lambda$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
$\mathcal{N}$ & 1 & 21.9 & $<0.001$ & 12.1 & 0.002 & -299.5 & (0.98, 2.67) & $\left( \begin{array}{cc}0.72 & 0.02 \\ 0.02 & 0.48 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 2 & 8.6 & 0.005 & 17.6 & $<0.001$ & -286.9 & (0.33, 2.59) & $\left( \begin{array}{cc}0.81 & -0.05 \\ -0.05 & 0.48 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -286.9 & (1.26, 2.70) & $\left( \begin{array}{cc}0.81 & 0.03 \\ -0.05 & 0.48 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{N}$ & 3 & \textcolor{red}{1.2} & 0.215 & 28.9 & $<0.001$ & -277.2 & (0.94, 2.74) & $\left( \begin{array}{cc}0.62 & 0.13 \\ 0.13 & 0.51 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -277.2 & (-0.81, 2.85) & $\left( \begin{array}{cc}0.62 & 0.11 \\ 0.13 & 0.52 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -277.2 & (1.30, 2.55) & $\left( \begin{array}{cc}0.62 & -0.06 \\ 0.13 & 0.38 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{SN}$ & 1 & 5.8 & 0.022 & 2.3 & 0.216 & -289.5 & (1.77, 2.66) & $\left( \begin{array}{cc}1.06 & 0.01 \\ 0.01 & 0.48 \end{array} \right)$ & (-2.76, 0.10) \\
\hline
$\mathcal{SN}$ & 2 & 9.7 & 0.003 & 31.2 & $<0.001$ & -283.5 & (0.78, 2.24) & $\left( \begin{array}{cc}0.90 & -0.15 \\ -0.15 & 0.56 \end{array} \right)$ & (-1.35, 1.12) \\
 &  &  &  &  &  & -283.5 & (1.04, 2.31) & $\left( \begin{array}{cc}0.90 & 0.09 \\ -0.15 & 0.61 \end{array} \right)$ & (1.07, 1.70) \\
\hline
$\mathcal{SN}$ & 3 & 22.9 & $<0.001$ & 69.4 & $<0.001$ & -282.1 & (1.02, 2.51) & $\left( \begin{array}{cc}0.52 & 0.11 \\ 0.11 & 0.59 \end{array} \right)$ & (0.96, 2.26) \\
 &  &  &  &  &  & -282.1 & (0.17, 2.84) & $\left( \begin{array}{cc}0.52 & 0.02 \\ 0.11 & 0.59 \end{array} \right)$ & (-0.81, -0.81) \\
 &  &  &  &  &  & -282.1 & (0.93, 2.67) & $\left( \begin{array}{cc}0.52 & -0.10 \\ 0.11 & 0.43 \end{array} \right)$ & (1.09, -1.62) \\
\hline
$\mathcal{T}$ & 1 & 10.4 & 0.002 & 3.8 & 0.102 & -292.8 & (1.04, 2.65) & $\left( \begin{array}{cc}0.61 & 0.01 \\ 0.01 & 0.41 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 2 & 4.7 & 0.037 & 16.8 & $<0.001$ & -283.9 & (1.25, 2.69) & $\left( \begin{array}{cc}0.42 & 0.01 \\ 0.01 & 0.41 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -283.9 & (0.28, 2.56) & $\left( \begin{array}{cc}0.42 & -0.06 \\ 0.01 & 0.40 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{T}$ & 3 & \textcolor{red}{0.0} & 0.392 & 30.8 & $<0.001$ & -275.6 & (0.94, 2.71) & $\left( \begin{array}{cc}0.57 & 0.10 \\ 0.10 & 0.45 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -275.6 & (-0.81, 2.90) & $\left( \begin{array}{cc}0.57 & 0.09 \\ 0.10 & 0.36 \end{array} \right)$ & \ldots \\
 &  &  &  &  &  & -275.6 & (1.39, 2.52) & $\left( \begin{array}{cc}0.57 & -0.07 \\ 0.10 & 0.36 \end{array} \right)$ & \ldots \\
\hline
$\mathcal{ST}$ & 1 & \textcolor{red}{0.4} & 0.321 & \textcolor{red}{0.0} & 0.681 & -285.8 & (1.63, 2.61) & $\left( \begin{array}{cc}0.84 & -0.01 \\ -0.01 & 0.42 \end{array} \right)$ & (-1.89, 0.20) \\
\hline
$\mathcal{ST}$ & 2 & 9.9 & 0.003 & 34.4 & $<0.001$ & -282.5 & (0.98, 2.32) & $\left( \begin{array}{cc}0.84 & -0.12 \\ -0.12 & 0.44 \end{array} \right)$ & (-1.54, 0.71) \\
 &  &  &  &  &  & -282.5 & (1.12, 2.45) & $\left( \begin{array}{cc}0.84 & 0.04 \\ -0.12 & 0.50 \end{array} \right)$ & (1.06, 1.24) \\
\hline
$\mathcal{ST}$ & 3 & 13.5 & $<0.001$ & 63.1 & $<0.001$ & -276.4 & (1.08, 2.56) & $\left( \begin{array}{cc}0.48 & 0.03 \\ 0.03 & 0.46 \end{array} \right)$ & (0.83, 2.76) \\
 &  &  &  &  &  & -276.4 & (0.94, 2.47) & $\left( \begin{array}{cc}0.48 & -0.09 \\ 0.03 & 0.14 \end{array} \right)$ & (3.65, -3.48) \\
 &  &  &  &  &  & -276.4 & (0.57, 2.50) & $\left( \begin{array}{cc}0.48 & -0.14 \\ 0.03 & 0.44 \end{array} \right)$ & (-4.76, -5.61) \\
\hline
\noalign{\smallskip}
\end{tabular}
$$
\end{table}
\twocolumn



==> tables/table_sim.tex <==
\begin{table}
\caption[]{Information criteria for the the samples generated using the Jackknife technique with 10\% and 30\% of the sample omitted and the Bootstrap method. 
See Section~\ref{sec:validation} for details. 
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) colour. 
The models that are suitable within the IC uncertainties (standard deviations of the generated samples) are shown
in green.
Cl. provides the number of GRB classes, $n$ shows the number of points in the generated data set, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:sim}
$$ 
\begin{tabular}{lllll}
\hline
\noalign{\smallskip}
Distr. & Cl. & $n$ & IC type & IC value \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

\multicolumn{5}{c}{Jackknife 10\%} \\
\hline
$\mathcal{N}$ & 1 & 368 & AIC & $1198.2 \pm 13.0$ \\
$\mathcal{N}$ & 2 & 368 & AIC & $\textcolor{ForestGreen}{1162.7 \pm 12.9}$ \\
$\mathcal{N}$ & 3 & 368 & AIC & $\textcolor{ForestGreen}{1164.8 \pm 12.7}$ \\
\hline
$\mathcal{SN}$ & 1 & 368 & AIC & $\textcolor{red}{1156.9 \pm 12.9}$ \\
$\mathcal{SN}$ & 2 & 368 & AIC & $\textcolor{ForestGreen}{1166.9 \pm 12.9}$ \\
$\mathcal{SN}$ & 3 & 368 & AIC & $\textcolor{ForestGreen}{1172.1 \pm 13.1}$ \\
\hline
$\mathcal{N}$ & 1 & 368 & BIC & $1217.8 \pm 12.9$ \\
$\mathcal{N}$ & 2 & 368 & BIC & $\textcolor{ForestGreen}{1205.7 \pm 12.9}$ \\
$\mathcal{N}$ & 3 & 368 & BIC & $1231.2 \pm 12.7$ \\
\hline
$\mathcal{SN}$ & 1 & 368 & BIC & $\textcolor{red}{1184.3 \pm 12.9}$ \\
$\mathcal{SN}$ & 2 & 368 & BIC & $1225.5 \pm 12.9$ \\
$\mathcal{SN}$ & 3 & 368 & BIC & $1262.0 \pm 13.1$ \\
\hline
\multicolumn{5}{c}{Jackknife 30\%}\\
\hline
$\mathcal{N}$ & 1 & 286 & AIC & $\textcolor{ForestGreen}{930.0 \pm 21.6}$ \\
$\mathcal{N}$ & 2 & 286 & AIC & $\textcolor{ForestGreen}{904.3 \pm 21.4}$ \\
$\mathcal{N}$ & 3 & 286 & AIC & $\textcolor{ForestGreen}{907.3 \pm 21.8}$ \\
\hline
$\mathcal{SN}$ & 1 & 286 & AIC & $\textcolor{red}{898.6 \pm 21.6}$ \\
$\mathcal{SN}$ & 2 & 286 & AIC & $\textcolor{ForestGreen}{908.1 \pm 21.0}$ \\
$\mathcal{SN}$ & 3 & 286 & AIC & $\textcolor{ForestGreen}{914.0 \pm 21.1}$ \\
\hline
$\mathcal{N}$ & 1 & 286 & BIC & $\textcolor{ForestGreen}{948.3 \pm 21.6}$ \\
$\mathcal{N}$ & 2 & 286 & BIC & $\textcolor{ForestGreen}{944.5 \pm 21.4}$ \\
$\mathcal{N}$ & 3 & 286 & BIC & $969.5 \pm 21.8$ \\
\hline
$\mathcal{SN}$ & 1 & 286 & BIC & $\textcolor{red}{924.2 \pm 21.6}$ \\
$\mathcal{SN}$ & 2 & 286 & BIC & $\textcolor{ForestGreen}{962.9 \pm 21.0}$ \\
$\mathcal{SN}$ & 3 & 286 & BIC & $998.1 \pm 21.1$ \\
\hline
\multicolumn{5}{c}{Bootstrap}\\
\hline
$\mathcal{N}$ & 1 & 409 & AIC & $\textcolor{ForestGreen}{1329.7 \pm 38.3}$ \\
$\mathcal{N}$ & 2 & 409 & AIC & $\textcolor{ForestGreen}{1282.8 \pm 36.3}$ \\
$\mathcal{N}$ & 3 & 409 & AIC & $\textcolor{red}{1276.5 \pm 36.4}$ \\
\hline
$\mathcal{SN}$ & 1 & 409 & AIC & $\textcolor{ForestGreen}{1281.2 \pm 36.0}$ \\
$\mathcal{SN}$ & 2 & 409 & AIC & $\textcolor{ForestGreen}{1283.4 \pm 35.8}$ \\
$\mathcal{SN}$ & 3 & 409 & AIC & $\textcolor{red}{1277.6 \pm 38.3}$ \\
\hline
$\mathcal{N}$ & 1 & 409 & BIC & $\textcolor{ForestGreen}{1349.8 \pm 38.3}$ \\
$\mathcal{N}$ & 2 & 409 & BIC & $\textcolor{ForestGreen}{1327.0 \pm 36.2}$ \\
$\mathcal{N}$ & 3 & 409 & BIC & $\textcolor{ForestGreen}{1344.7 \pm 36.4}$ \\
\hline
$\mathcal{SN}$ & 1 & 409 & BIC & $\textcolor{red}{1309.3 \pm 36.0}$ \\
$\mathcal{SN}$ & 2 & 409 & BIC & $\textcolor{ForestGreen}{1343.7 \pm 35.8}$ \\
$\mathcal{SN}$ & 3 & 409 & BIC & $\textcolor{ForestGreen}{1369.9 \pm 38.3}$ \\
\hline

\noalign{\smallskip}
\end{tabular}
$$ 
\end{table}

==> tables/table_sim_err.tex <==
\begin{table}
\caption[]{Information criteria for the the samples generated using the uncertainties of the rest-frame $T_{90}$ and $E_p$. 
See Section~\ref{sec:validation} for details. 
The acceptable models are shown in red ($\Delta \textrm{IC} < 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) colour. 
The models that are suitable within the IC uncertainties (standard deviations of the generated sample), are shown in green.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:sim_err}

\begin{tabular}{lccc}
\hline
\noalign{\smallskip}
Distr. & Cl. & AIC & BIC \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

$\mathcal{N}$ & 1 & $1356.8 \pm 19.2$ & $\textcolor{ForestGreen}{1376.9 \pm 19.3}$ \\
$\mathcal{N}$ & 2 & $\textcolor{blue}{1316.8 \pm 17.3}$ & $\textcolor{ForestGreen}{1360.9 \pm 17.3}$ \\
$\mathcal{N}$ & 3 & $\textcolor{ForestGreen}{1320.1 \pm 16.9}$ & $1388.3 \pm 16.9$ \\
\hline
$\mathcal{SN}$ & 1 & $\textcolor{red}{1314.1 \pm 18.5}$ & $\textcolor{red}{1342.2 \pm 18.5}$ \\
$\mathcal{SN}$ & 2 & $\textcolor{ForestGreen}{1321.0 \pm 17.0}$ & $1381.2 \pm 17.0$ \\
$\mathcal{SN}$ & 3 & $\textcolor{ForestGreen}{1327.2 \pm 16.6}$ & $1419.5 \pm 16.6$ \\
\hline
$\mathcal{T}$ & 1 & $1355.8 \pm 16.5$ & $1379.9 \pm 16.5$ \\
$\mathcal{T}$ & 2 & $\textcolor{ForestGreen}{1319.1 \pm 17.1}$ & $\textcolor{ForestGreen}{1367.3 \pm 17.1}$ \\
$\mathcal{T}$ & 3 & $\textcolor{ForestGreen}{1322.2 \pm 16.7}$ & $1394.5 \pm 16.7$ \\
\hline
$\mathcal{ST}$ & 1 & $\textcolor{red}{1315.1 \pm 16.6}$ & $\textcolor{ForestGreen}{1347.2 \pm 16.6}$ \\
$\mathcal{ST}$ & 2 & $\textcolor{ForestGreen}{1324.1 \pm 17.1}$ & $1388.3 \pm 17.1$ \\
$\mathcal{ST}$ & 3 & $\textcolor{ForestGreen}{1329.7 \pm 17.0}$ & $1426.0 \pm 17.0$ \\
\hline

\noalign{\smallskip}
\end{tabular}
\end{table}

==> tables/table_snr.tex <==
\begin{table}
\caption[]{Information criteria for the rest-frame distributions with 10\% of the dimmest bursts excluded. The acceptable models are shown in red ($\Delta \textrm{IC}< 2$) and blue ($2 < \Delta \textrm{AIC} < 4$) colour.
Cl. provides the number of GRB classes, $\mathcal{N}$ ($\mathcal{SN}$) and $\mathcal{T}$ ($\mathcal{ST}$) denote the symmetric (skewed) Gaussian and Student distributions, correspondingly.}
\label{tab:snr}
$$ 
 \begin{tabular}{llrrrrr}
 
    \hline
    \noalign{\smallskip}
    Statistics & Cl. & Sample & $\Delta_\textrm{AIC}$ & $w_i$ (AIC) & $\Delta_\textrm{BIC}$ & $w_i$ (BIC) \\
    \noalign{\smallskip}
    \hline
    \noalign{\smallskip}
    
$\mathcal{N}$ & 1 & Total & 44.7 & $<0.001$ & 36.8 & $<0.001$ \\
$\mathcal{N}$ & 2 & Total & 5.7 & 0.040 & 21.3 & $<0.001$ \\
$\mathcal{N}$ & 3 & Total & 8.9 & 0.008 & 47.9 & $<0.001$ \\
\hline
$\mathcal{SN}$ & 1 & Total & \textcolor{red}{0.0} & 0.692 & \textcolor{red}{0.0} & 0.953 \\
$\mathcal{SN}$ & 2 & Total & 10.3 & 0.004 & 41.5 & $<0.001$ \\
$\mathcal{SN}$ & 3 & Total & 16.8 & $<0.001$ & 79.2 & $<0.001$ \\
\hline
$\mathcal{T}$ & 1 & Total & 45.4 & $<0.001$ & 41.5 & $<0.001$ \\
$\mathcal{T}$ & 2 & Total & 8.4 & 0.010 & 27.9 & $<0.001$ \\
$\mathcal{T}$ & 3 & Total & 10.7 & 0.003 & 53.6 & $<0.001$ \\
\hline
$\mathcal{ST}$ & 1 & Total & \textcolor{blue}{2.1} & 0.242 & 6.0 & 0.047 \\
$\mathcal{ST}$ & 2 & Total & 14.6 & $<0.001$ & 49.8 & $<0.001$ \\
$\mathcal{ST}$ & 3 & Total & 19.2 & $<0.001$ & 85.6 & $<0.001$ \\
\hline
\hline
$\mathcal{N}$ & 1 & KW trig & 20.2 & $<0.001$ & 13.9 & 0.001 \\
$\mathcal{N}$ & 2 & KW trig & \textcolor{red}{0.8} & 0.252 & 13.4 & 0.001 \\
$\mathcal{N}$ & 3 & KW trig & \textcolor{blue}{3.7} & 0.059 & 35.3 & $<0.001$ \\
\hline
$\mathcal{SN}$ & 1 & KW trig & \textcolor{red}{0.0} & 0.375 & \textcolor{red}{0.0} & 0.915 \\
$\mathcal{SN}$ & 2 & KW trig & 4.6 & 0.038 & 29.9 & $<0.001$ \\
$\mathcal{SN}$ & 3 & KW trig & 7.0 & 0.011 & 57.6 & $<0.001$ \\
\hline
$\mathcal{T}$ & 1 & KW trig & 19.8 & $<0.001$ & 16.7 & $<0.001$ \\
$\mathcal{T}$ & 2 & KW trig & \textcolor{blue}{3.2} & 0.076 & 19.0 & $<0.001$ \\
$\mathcal{T}$ & 3 & KW trig & 6.2 & 0.017 & 41.0 & $<0.001$ \\
\hline
$\mathcal{ST}$ & 1 & KW trig & \textcolor{red}{1.7} & 0.160 & 4.8 & 0.083 \\
$\mathcal{ST}$ & 2 & KW trig & 7.2 & 0.010 & 35.7 & $<0.001$ \\
$\mathcal{ST}$ & 3 & KW trig & 11.0 & 0.002 & 64.7 & $<0.001$ \\
\hline
\hline
$\mathcal{N}$ & 1 & KW \& BAT & \textcolor{red}{0.0} & 0.451 & \textcolor{red}{0.0} & 0.943 \\
$\mathcal{N}$ & 2 & KW \& BAT & \textcolor{red}{1.5} & 0.213 & 19.6 & $<0.001$ \\
$\mathcal{N}$ & 3 & KW \& BAT & 5.0 & 0.037 & 41.2 & $<0.001$ \\
\hline
$\mathcal{SN}$ & 1 & KW \& BAT & 4.3 & 0.053 & 10.4 & 0.005 \\
$\mathcal{SN}$ & 2 & KW \& BAT & 7.8 & 0.009 & 38.0 & $<0.001$ \\
$\mathcal{SN}$ & 3 & KW \& BAT & 13.4 & 0.001 & 67.7 & $<0.001$ \\
\hline
$\mathcal{T}$ & 1 & KW \& BAT & \textcolor{blue}{2.8} & 0.111 & 5.8 & 0.052 \\
$\mathcal{T}$ & 2 & KW \& BAT & 4.3 & 0.053 & 25.4 & $<0.001$ \\
$\mathcal{T}$ & 3 & KW \& BAT & 4.2 & 0.055 & 43.4 & $<0.001$ \\
\hline
$\mathcal{ST}$ & 1 & KW \& BAT & 6.8 & 0.015 & 15.9 & $<0.001$ \\
$\mathcal{ST}$ & 2 & KW \& BAT & 10.3 & 0.003 & 43.5 & $<0.001$ \\
$\mathcal{ST}$ & 3 & KW \& BAT & 15.5 & $<0.001$ & 72.8 & $<0.001$ \\
\hline
\hline
$\mathcal{N}$ & 1 & GBM all & 18.7 & $<0.001$ & 10.8 & 0.003 \\
$\mathcal{N}$ & 2 & GBM all & 6.0 & 0.031 & 16.2 & $<0.001$ \\
$\mathcal{N}$ & 3 & GBM all & 11.7 & 0.002 & 40.0 & $<0.001$ \\
\hline
$\mathcal{SN}$ & 1 & GBM all & 5.4 & 0.041 & 3.5 & 0.101 \\
$\mathcal{SN}$ & 2 & GBM all & 7.8 & 0.012 & 30.1 & $<0.001$ \\
$\mathcal{SN}$ & 3 & GBM all & 20.4 & $<0.001$ & 66.8 & $<0.001$ \\
\hline
$\mathcal{T}$ & 1 & GBM all & 4.9 & 0.053 & \textcolor{red}{0.0} & 0.579 \\
$\mathcal{T}$ & 2 & GBM all & \textcolor{blue}{3.7} & 0.097 & 16.9 & $<0.001$ \\
$\mathcal{T}$ & 3 & GBM all & \textcolor{blue}{3.1} & 0.131 & 34.4 & $<0.001$ \\
\hline
$\mathcal{ST}$ & 1 & GBM all & \textcolor{red}{0.0} & 0.615 & \textcolor{red}{1.2} & 0.318 \\
$\mathcal{ST}$ & 2 & GBM all & 7.0 & 0.019 & 32.3 & $<0.001$ \\
$\mathcal{ST}$ & 3 & GBM all & 26.5 & $<0.001$ & 75.9 & $<0.001$ \\

\hline

\noalign{\smallskip}
\end{tabular}
$$ 
\end{table}
